Conformal-DP: A Density-Aware Mechanism for Differential Privacy over Riemannian Manifolds via Conformal Transformation

Differential Privacy (DP) is being increasingly adopted for non-Euclidean data that lie on complex, high-dimensional manifolds. Existing DP mechanisms for manifold data consider geometric properties when calibrating privacy perturbations, but they largely fail to capture variations in data density within datasets, leading to biased perturbations and suboptimal privacy-utility trade-offs due to heterogeneous data distributions. In this paper, we propose a novel density-aware differential privacy mechanism on Riemannian manifolds, referred to as Conformal-DP, that leverages conformal transformations to calibrate perturbations based on local densities and to induce a density-balanced geometry. We prove that our mechanism satisfies $\epsilon$-differential privacy on any complete Riemannian manifold under mild regularity assumptions. In addition, we derive a closed-form expected geodesic error bound that depends only on the underlying data density ratio and is independent of global curvature. Our empirical results on synthetic and real-world datasets demonstrate that the proposed Conformal-DP mechanism substantially improves the privacy-utility trade-off in heterogeneous data distribution settings, with worst-case performance comparable to state-of-the-art manifold DP mechanisms that assume uniformly distributed data.

==> algorithms.tex <==
% \begin{algorithm}[b!]
% \label{alg:1}
% \caption{Compute Conformal Fréchet Mean via Riemannian Gradient Descent}

% \begin{algorithmic}[1]
% \State \textbf{Input:} Dataset $D = \{x_1,...,x_n\} \subset \mathcal{M}$, initial point $x^{(0)}$ (e.g., empirical mean), step size strategy $\alpha_k$, maximum iteration $k_{\text{max}}$, stopping criterion $\delta$
% \State \textbf{Output:} Conformal Fréchet mean $\eta(D) \approx x^{\left(k_{\max }\right)}$

% \State \textbf{Initialization:} 
% \State \quad Set current point $x \leftarrow x^{(0)}$, iteration count $k \leftarrow 0$

% \State \textbf{Iterative Optimization:}
% \While{$k < k_{\text{max}}$ \textbf{and} $\|\nabla F^*(x)\| \geq \delta$}
%     \State Compute gradient:
%     \[
%     \nabla F^*(x) = \frac{1}{n} \sum_{i=1}^n \rho_g^2(x, x_i) \left[ -\log_x^{(g^*)}(x_i) \right]
%     \]
%     \If{$\|\nabla F^*(x)\| < \delta$}
%         \State \textbf{break}
%     \EndIf
%     \State Select step size $\alpha_k$
%     \State Update point via exponential map:
%     \[
%     x^{k+1} \leftarrow \exp_{x^k}^{(g^*)}\left( -\alpha_k \cdot \nabla F^*(x^k) \right)
%     \]
%     \State Increment iteration: $k \leftarrow k + 1$
% \EndWhile

% \State \textbf{Return:} $\eta(D)$
% \end{algorithmic}
% \end{algorithm}


\begin{algorithm}[H]
\caption{Differentially Private Conformal Laplace Sampling on Manifolds}
\label{alg:mcmc}

\begin{algorithmic}[1]
\State \textbf{Input:} 
\State \quad Non-private statistic $\eta_{\mathrm{np}}(D)$ (e.g., Fréchet mean under $g$),
\State \quad Privacy budget $\varepsilon > 0$, 
\State \quad Global sensitivity bound $\Delta^*_{\mathrm{global}}=\sqrt{\overline{\phi}}\,\Delta$ (data-independent),
\State \quad Volume term $\varepsilon_{\mathrm{vol}}=\tfrac{n}{2}\ln(\overline{\phi}/\underline{\phi})$,
\State \quad Proposal kernel $Q(\cdot\,|\,\cdot)$ with public step $r_0$ (for proposals only),
\State \quad Maximum iterations $T_{\text{max}}$

\State \textbf{Output:} 
\State \quad Differentially private sample $Z$ from $\mathbb{P}^*(z \mid \eta_{\mathrm{np}}(D), \lambda^*)$ (full support on $\mathcal{M}$)

\State \textbf{Step 1: Calculate Noise Intensity}
\[
\lambda^* \leftarrow \min\!\left\{\frac{\varepsilon-\varepsilon_{\mathrm{vol}}}{2\,\Delta^*}, \;\lambda_{\max}\right\}
\quad \text{(Default: } \lambda^* = \frac{\varepsilon-\varepsilon_{\mathrm{vol}}}{2\,\Delta^*}\text{)}
\]

\State \textbf{Step 2: Select Sampling Method}
\If{\textbf{MH \cite{metropolis1949monte}}}
    \State Initialize $z^{(0)} \leftarrow \eta_{\mathrm{np}}(D)$ (or any $z^{(0)}\!\in\! M$) \Comment{Starting point; no hard truncation}
    \For{$t = 0$ \textbf{to} $T_{\text{max}}-1$}
        \State Propose $z' \sim Q(\cdot \mid z^{(t)})$ \Comment{e.g., uniform on $B^{g^*}_{r_0}(z^{(t)})$ with public $r_0$}
        \State Compute acceptance ratio (density w.r.t.\ $\mu_g$):
        \[
        \alpha \leftarrow 
        \frac{\exp\!\left[-\lambda^* \rho_{g^*}(\eta_{\mathrm{np}}(D), z')\right]\;\phi(z')^{\frac{n}{2}}\; Q(z^{(t)} \mid z')}
             {\exp\!\left[-\lambda^* \rho_{g^*}(\eta_{\mathrm{np}}(D), z^{(t)})\right]\;\phi(z^{(t)})^{\frac{n}{2}}\; Q(z' \mid z^{(t)})}
        \]
        \State Accept $z^{(t+1)} \leftarrow z'$ with probability $\min(1, \alpha)$
    \EndFor
    \State Set $Z \leftarrow z^{(T_{\text{max}})}$ \Comment{Final sample}
\Else \Comment{Semi-analytic method for specific manifolds}
    \State Exploit manifold structure (e.g., sphere, hyperbolic space)
    \State Directly sample from $\mathbb{P}^* (z \mid \eta_{\mathrm{np}}(D), \lambda^*)$ (full support on $\mathcal{M}$)

\EndIf

\State \textbf{Return:} $Z$ \Comment{$\varepsilon$-DP perturbed output}
\end{algorithmic}
\end{algorithm}





==> header.tex <==
\usepackage{amsthm}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{textcomp}
\usepackage[x11names,dvipsnames]{xcolor}
\newcommand{\rev}[1]{\textcolor{red}{#1}}
\usepackage{booktabs}
\usepackage{subcaption} 
\usepackage{diagbox}
\usepackage{float}
\usepackage{makecell} % for \thickhline
\usepackage{array}
\usepackage{svg}
\usepackage{epstopdf}
\usepackage{authblk}
\usepackage{soul}
\usepackage{pifont}
\usepackage{xr-hyper}
\usepackage[hidelinks]{hyperref}
% \usepackage{hyperref}
% \hypersetup{
%     colorlinks=true,
%     linkcolor=blue,
%     citecolor=blue,
%     urlcolor=blue
% }
\usepackage[capitalize,noabbrev]{cleveref}
% *** SPECIALIZED LIST PACKAGES ***
%
% \usepackage{algorithmic} 
\usepackage{algorithm}
\usepackage{algorithmic}
% *** ALIGNMENT PACKAGES ***
%
\usepackage{array}
% *** SUBFIGURE PACKAGES ***
% \ifCLASSOPTIONcompsoc
%  \usepackage[caption=false,font=footnotesize,labelfont=sf,textfont=sf]{subfig}
% \else
%  \usepackage[caption=false,font=footnotesize]{subfig}
% \fi
\usepackage{url}
\newcommand{\orcidlink}[1]{%
  \textsuperscript{\href{https://orcid.org/#1}{\includegraphics[width=1.6ex]{orcid.png}}}%
}
% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}
% ============================================================================================
% ============================================================================================
% Plain-style environments (with italic body text)
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]      % Theorem 1.1, 1.2, etc.
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
% Definition-style environments (with normal text)
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
% Remark-style environments (unnumbered)
\theoremstyle{remark}
\newtheorem*{remark}{Remark}

\newcommand{\parhead}[1]{\vspace{3pt plus 1pt minus 1pt}\par\noindent\textbf{#1}\hspace{.4em plus .2em minus .2em}}
\renewcommand{\paragraph}[1]{\parhead{#1}}



\def\OJlogo{\vspace{-4pt}$<$Society logo(s) and publication title will appear here.$>$}
\def\seclogo{\vspace{10pt}$<$Society logo(s) and publication title will appear here.$>$}

\def\authorrefmark#1{\ensuremath{^{\textbf{#1}}}}

\newcommand{\aref}[1]{\ref{A-#1}} % main里引用full里的appendix标签
\newcommand{\mref}[1]{\ref{M-#1}} % appendix里引用full里的main标签
\newcommand{\acref}[1]{\cref{A-#1}}
\newcommand{\mcref}[1]{\cref{M-#1}}
